SAM3D-Guided Object-Centric Representation Alignment for Vision-Language-Action Models

Vision-Language-Action (VLA) models have shown strong potential for general robot manipulation, but most existing models rely on 2D visual-language backbones and lack fine-grained 3D understanding of target objects, especially under occlusion, pose variation, scale changes, and precise spatial interaction. We propose an object-centric 3D representation alignment framework built upon $\pi_0$, using SAM3D as a frozen 3D teacher to provide target-object 3D priors during training. Specifically, we localize task-relevant objects with object recognition models, generate corresponding object masks, and use SAM3D to extract dense object-level 3D representations, which are aligned with intermediate visual features of $\pi_0$. This enables the policy to internalize target-object 3D information while preserving the original RGB-language-to-action inference pipeline without requiring depth, point clouds, masks, SAM3D, or additional 3D modules at test time. Simulation experiments show consistent improvements, achieving 99.1\% on LIBERO and an average length of 4.11 on CALVIN. Real-world experiments further demonstrate that our method is particularly effective in long-horizon manipulation scenarios where the robot must focus on different target objects across multiple subtasks.

==> corl_2026_template_cameraready/supplyment.tex <==
```latex
\paragraph{Choice of Alignment Layer.}
We further analyze which VLA layer is more suitable for SAM3D-guided feature alignment. Our \(\pi_0\) VLM backbone contains 18 causal attention layers. As shown in Fig.~X, shallow layers already show some attention to the target object, but their responses are still mixed with low-level visual cues and local texture patterns. More importantly, if the alignment is applied to very shallow layers, the injected object-centric 3D information has to pass through many subsequent transformer layers, where it may be weakened or overwritten during visual-language and action-related feature fusion. Therefore, shallow-layer supervision may not be effectively preserved in the final policy representation.

On the other hand, the last layers are closer to action prediction and language-conditioned decision making. At this stage, visual and language features tend to become more modality-agnostic, and part of the vision-specific spatial details may be lost. We therefore choose the 11th layer as the alignment layer, which provides a good trade-off between target-object awareness and vision-specific representation. This layer shows more concentrated attention on the task-relevant object while still preserving sufficient spatial visual information, making it suitable for SAM3D object-centric supervision.
```

